The limits of min-max optimization algorithms: convergence to spurious non-critical sets

Compared to ordinary function minimization problems, min-max optimization algorithms encounter far greater challenges because of the existence of periodic cycles and similar phenomena. Even though some of these behaviors can be overcome in the convex-concave regime, the general case is considerably more difficult. On that account, we take an in-depth look at a comprehensive class of state-of-the art algorithms and prevalent heuristics in non-convex / non-concave problems, and we establish the following general results: a) generically, the algorithms' limit points are contained in the ICT sets of a common, mean-field system; b) the attractors of this system also attract the algorithms in question with arbitrarily high probability; and c) all algorithms avoid the system's unstable sets with probability 1. On the surface, this provides a highly optimistic outlook for min-max algorithms; however, we show that there exist spurious attractors that do not contain any stationary points of the problem under study. In this regard, our work suggests that existing min-max algorithms may be subject to inescapable convergence failures. We complement our theoretical analysis by illustrating such attractors in simple, two-dimensional, almost bilinear problems.

==> App-Errata.tex <==
%----------------------------------------------------------------------
%%% APP: ERRATA
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


Put here any errata we find:
\begin{enumerate}
\item
Fix \eqref{eq:variance} or \cref{asm:noise} [\eqref{eq:variance} is probably easier.]
\end{enumerate}

==> Impact.tex <==
%----------------------------------------------------------------------
%%% IMPACT
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


This is a theoretical work which does not present any foreseeable societal consequence.

==> Temp.tex <==
Now, if by continuity, there exists a compact neighborhood
%We break the proof into three steps.
%
%\para{Controlling the martingale error}
%Fix some $\eps > 0$.
%As in the proof of \cref{thm:global}, let $\noise_{\run} = \nabla\lyap(\state_{\run}) - \nabla\sobj(\state_{\run};\sample_{\run})$ and set $\snoise_{\run} = \braket{\noise_{\run}}{\state_{\run}-\sol}$ where $\sol\in\cpt$ is such that \eqref{eq:LVC} holds as an equality only if $\point\in\cpt$ (cf.~\cref{def:VC-local}).
%We show below that there exists a step-size sequence $(\step_{\run})_{\run=\start}^{\infty}$ such that
%\begin{equation}
%\label{eq:mg_noise_bound}
%\probof*{\sup_{\run} \sum_{\runalt=\start}^{\run} \step_{\runalt} \snoise_{\runalt} \leq \eps} \geq 1 - \frac{\delta}{2}.
%\end{equation}
%To show this, we start by noting that, as in the proof of \cref{prop:recurrence}, the aggregate process $S_{\run} = \sum_{\runalt=\start}^{\run} \step_{\runalt} \snoise_{\runalt}$ is a martingale relative to the natural filtration $\filter_{\run}$ of $\sample_{\run}$.
%Then, letting $R= \sup_{\point\in\points} \norm{\point}$, we can bound the variance of each individual term of $S_{\run}$ as follows:
%\begin{flalign}
%\label{eq:MSE_local1}
%\exof{\snoise_{\runalt}^{2}}
%	&= \exof{\exof{\abs{\braket{\noise_{\runalt}}{\state_{\runalt} - \sol}}^{2} \given \filter_{\runalt-1}}}
%	\notag\\
%	&\leq \exof{\exof{\dnorm{\noise_{\runalt}}^{2} \norm{\state_{\runalt} - \sol}^{2} \given \filter_{\runalt-1}}}
%	\notag\\
%	&= \exof{\norm{\state_{\runalt} - \sol}^{2} \exof{\dnorm{\noise_{\runalt}}^{2} \given \filter_{\runalt-1}}}
%	\notag\\
%	&\leq R^{2} \vbound^{2},
%\end{flalign}
%where the first inequality follows from the definition of the dual norm
%%the second equality follows from $\state_{\runalt}$ is adapted to $\filter_{\runalt}$
%and the second one follows from \eqref{eq:MSE}. Consequently, by Doob's maximal inequality (\cref{thm:mg_convergence4} in \cref{app:aux}), we have:
%\begin{equation}
%\label{eq:MSE_local2}
%\probof*{\sup_{0\leq \runalt \leq \run} S_{\runalt} \geq \eps}
%	\leq \probof*{\sup_{0\leq \runalt \leq \run} |S_{\runalt}| \geq \eps}
%	\leq \frac{\exof{S_{\run}^{2}}}{\eps^{2}}
%	\leq \frac{R^{2} \vbound^{2} \sum_{\runalt=\start}^{\run} \step_{\runalt}^{2}}{\eps^{2}},
%	\end{equation}
%where the last inequality follows from expanding $\exof{\abs{S_{\run}}^{2}}$, using \cref{eq:MSE_local1}, and noting that $\exof{\snoise_{\runalt}\snoise_{\ell}} = \exof{\exof{\snoise_{\runalt} \snoise_{\ell}} \given \filter_{\runalt\vee\ell-1}} = 0$ whenever $\runalt\neq\ell$.
%Therefore, by picking $\step_{\run}$ so that $\sum_{\runalt=\start}^{\infty} \step_{\runalt}^{2} \leq \eps^{2}\delta/(2R^{2}\vbound^{2})$, \cref{eq:MSE_local2} gives
%\begin{equation}
%\label{eq:MSE_local3}
%\probof*{\sup_{0\leq k \leq t} S_{\runalt} \geq \eps}
%	\leq \frac{R^{2} \vbound^{2} \sum_{\runalt=\start}^{\run} \step_{\runalt}^{2}}{\eps^{2}}
%	\leq \frac{R^{2} \vbound^{2} \sum_{\runalt=\start}^{\infty} \step_{\runalt}^{2}}{\eps^{2}}
%	\leq \frac{\delta}{2}
%	\quad
%	\text{for all $\run$}.
%\end{equation}
%Since the above holds for all $\run$, our assertion follows.
%
%
%\para{Controlling the submartingale error}
%Again, fix some $\eps > 0$ and, with a fair amount of foresight, let $R_{\run} = (2\strong)^{-1} \sum_{\runalt=\start}^{\run} \step_{\runalt}^{2} \dnorm{\est\payv_{\runalt}}^{2}$.
%By construction, $R_{\run}$ is a non-negative submartingale relative to $\filter_{\run}$.
%We again establish that there exists step-size sequence $(\step_{\run})_{\run=\start}^{\infty}$ satisfying the summability condition \eqref{eq:L2L1} and such that
%\begin{equation}
%\label{eq:smg_noise_bound}
%\probof*{\sup_{\run} R_{\run} \leq \eps}
%	\geq 1 - \frac{\delta}{2}.
%\end{equation}
%To show this, Doob's maximal inequality for submartingales (\cref{thm:mg_convergence3}) gives
%\begin{equation}
%\label{eq:prob-bound2}
%\probof*{\sup_{0 \leq \runalt \leq \run} R_{\runalt} \geq \eps} 
%	\leq \frac{\exof{R_{\run}}}{\eps}
%	\leq \frac{\vbound^{2} \sum_{\runalt=\start}^{\run} \step_{\runalt}^{2}}{2\strong\eps},
%	\end{equation}
%where we used the fact that $\exof{\cramped{\dnorm{\nabla\sobj(\state_{\run};\sample_{\run})}^{2}}} \leq \vbound^{2}$ for some finite $\vbound<\infty$.
%Consequently, if we choose $\step_{\run}$ so that $\sum_{\runalt=\start}^{\infty} \step_{\runalt}^{2} \leq \strong\delta\eps/\vbound^{2}$, \cref{eq:prob-bound2} readily gives
%\begin{equation}
%\probof*{\sup_{0 \leq \runalt \leq \run} R_{\runalt} \geq \eps}
%	\leq \frac{\vbound^{2} \sum_{\runalt=\start}^{\infty} \step_{\runalt}^{2}}{2\strong\eps}
%	\leq \frac{\delta}{2}
%	\quad
%	\text{for all $\run$}
%\end{equation}
%Since the above is true for all $\run$, \cref{eq:smg_noise_bound} follows.
%
%\para{Error aggregation}
%To combine the above, assume that $\eps>0$ is sufficiently small so that $\fball(\sol, 3\eps) \subset U$, where $U$ is the open neighborhood  given in \eqref{eq:LVC}.
%Furthermore, let $\nhd = \fball(\sol, \eps)$ and pick a step-size sequence $\step_{\run}$ satisfying \eqref{eq:L2L1} and such that
%\begin{equation}
%\label{eq:step-small}
%\sum_{\run=\start}^{\infty} \step_{\run}^{2}
%	\leq \min\braces*{\frac{\delta\eps^{2}}{2R^{2}\vbound^{2}}, \frac{\strong\delta\eps}{\vbound^{2}}}.
%\end{equation}
%If $\state_{\start}\in\nhd$, it follows that $\fench(\sol,\score_{\start}) < \eps$ by the definition of $\fball$ (cf.~\cref{def:metrics}).
%Then, by \cref{eq:mg_noise_bound,eq:smg_noise_bound}, we get $\probof{\sup_{\run} S_{\run} \geq \eps} \leq \delta/2$ and $\probof{\sup_{\run} R_{\run} \geq \eps} \leq \delta/2$.
%Consequently, with this choice of $\step_{\run}$, it follows that
%\begin{equation}
%\probof*{\sup\nolimits_{\run} \max\{S_{\run},R_{\run}\} \leq \eps}
%	\geq 1 - \delta/2 - \delta/2
%	= 1 - \delta
%\end{equation}
%Then, letting $\fench_{\run} = \fench(\sol,\score_{\run})$ and arguing as in the proof of \cref{thm:global}, we may expand $\fench_{\run} = \fench(\sol,\score_{\run})$ to get
%\begin{flalign}
%\label{eq:Dbound-stoch}
%\fench_{\run}
%	&= \fench(\sol, \score_{\run} + \step_{\run}\est\payv_{\run})
%	\notag\\
%%	& \leq \fench(\sol, \score_{\run})
%%	+ \step_{\run} \braket{\payv(\state_{\run}) + \noise_{\run}}{\mirror(\score_{\run}) - \sol}
%%	+ \frac{\step_{\run}^{2}}{2\strong} \dnorm{\payv(\state_{\run}) + \noise_{\run}}^{2}
%%	\notag\\
%	&\leq \fench_{\run}
%	+ \step_{\run} \braket{\payv(\state_{\run})}{\state_{\run} - \sol}
%	+ \step_{\run} \snoise_{\run}
%	%	+ \step_{\run} \bnoise_{\run}
%	+ \frac{\step_{\run}^{2}}{2\strong} \dnorm{\nabla\sobj(\state_{\run};\sample_{\run})}^{2}
%\end{flalign}
%with $\snoise_{\run} = \braket{\noise_{\run}}{\state_{\run}-\sol}$ defined as above.
%Telescoping \eqref{eq:Dbound-stoch} then yields
%\begin{flalign}
%\label{eq:Dbound-n}
%\fench_{\run}
%	&\leq \fench_{\start}
%	+ \sum_{\runalt=\start}^{\run} \step_{\runalt} \braket{\payv(\state_{\runalt})}{\state_{\runalt} - \sol}
%	+ S_{\run}
%	+ R_{\run}
%	\notag\\
%	%	+ \sum_{\runalt=\start}^{\run} \step_{\runalt}\bnoise_{\runalt}\\
%	&\leq \eps + \sum_{\runalt=\start}^{\run} \step_{\runalt}\braket{\payv(\state_{\runalt})}{\state_{\runalt} - \sol} + \eps + \eps,
%\end{flalign}
%with probability at least $1-\delta$.
%Therefore, with probability at least $1-\delta$, we have
%\begin{equation}
%\label{eq:Fench-maximal}
%\fench(\sol,\score_{\run})
%	\leq 3\eps + \sum_{\runalt=\start}^{\run} \step_{\runalt}\braket{\payv(\state_{\runalt})}{\state_{\runalt} - \sol}.
%\end{equation}
%
%Now, assume inductively that, for all $\runalt\leq\run$, we have $\fench(\sol,\score_{\runalt}) \leq 3\eps$ or, equivalently, $\state_{\runalt} \in \fball(\sol, 3\eps)$.
%In turn, this implies that $\braket{\payv(\state_{\runalt})}{\state_{\runalt} - \sol} \leq 0$ for all $\runalt\leq \run$, and hence, by \eqref{eq:Fench-maximal}, that $\fench(\sol,\score_{\run}) \leq 3\eps$ as well.
%Since the base case $\state_{\start} \in \nhd = \fball(\sol, \eps) \subset \fball(\sol, 3\eps)$ is satisfied automatically, we conclude that $\state_{\run}$ stays in $\fball(\sol, 3\eps) \subset U$ for all $\run$ with probability at least $1-\delta$.
%Our claim then follows by conditioning on this event and repeating the same steps as in the proof of \cref{thm:global}.


==> conclusion.tex <==
%----------------------------------------------------------------------
%%% CONCLUSION
%----------------------------------------------------------------------
% !TEX root = ./Main.tex
The generalized \ac{RM} template captures a wide array of existing min-max algorithms, and the machinery of stochastic approximation allows us to derive a series of new convergence results, desirable or undesirable. 

On the other hand, our framework leaves out several important settings that are of immediate interest to the machine learning practitioners. We discuss these below along with preliminary numerical results:

\begin{enumerate}
\item Instead of the ``moving average'' in \cref{lem:averaging}, one can take the \textbf{ergodic average} ($\curr[\state']= \frac{1}{n}\insum_{\runalt = 1}^\run \state_\runalt$) as is customary in convex-concave \eqref{eq:minmax} \cite{nemirovski2004prox,juditsky2011solving}. We plot one such trajectory in \cref{fig:spurious} (the blue curves). Evidently, we see that ergodic average can force the trajectories to halt at non-critical points, and this convergence is by no means min-max optimal.

\item Many recent works attempt to address the cycling behaviors of min-max algorithms via incorporating \textbf{second-order} oracles; see \cref{app:perturb} for a non-exhaustive list. In this regard, we have applied several popular {second-order} methods to \eqref{eq:perturbed-bilinear} and \eqref{eq:forsaken-stable} in \cref{app:perturb}. The result shows that these algorithms suffer similar symptoms as first-order algorithms in our examples.

\item Other than the diminishing step-sizes studied in this paper, another common strategy in practice is to simply set $\curr[\step]$ to a \textbf{constant step-size}. While our analysis does not cover this setting, there exist several techniques in stochastic approximation to boost from our ``almost surely'' statements for $\curr[\step]\searrow0$ to \emph{concentration} or \emph{high-probability} results when $\curr[\step] \equiv \step$ is small \cite{kushner1981asymptotic, KY97, Bor08}. %Extending our results to constant step-size rules thus present an immediate and promising future work.

For completeness, in \cref{app:const-step} we examine various constant step-size \ac{RM} schemes applied to \eqref{eq:perturbed-bilinear} and \eqref{eq:forsaken-stable}. The outcome coincides with our intuition that these schemes should concentrate around the spurious attracting \ac{ICT} sets, and hence exhibit similar (and problematic) behaviors as \ac{RM} schemes with $\curr[\step]\searrow0$; see \cref{fig:const-step}.


\item \textbf{Adaptive methods} such as Adam \cite{kingma2014adam} are ubiquitous in \acs{GAN} training. However, in \cref{app:adaptive} we report that they fail to solve the simple objectives \eqref{eq:perturbed-bilinear} and \eqref{eq:forsaken-stable}. Moreover, some methods even show a potentially detrimental tendency of converging to $\max-\min$ points, the opposite of desirable solutions; see \cref{fig:adaptive}.
%some worrisome behaviors of these algorithms applied to \eqref{eq:perturbed-bilinear} and \eqref{eq:forsaken-stable}.
\end{enumerate}






Finally, we should clarify that these preliminary discussions are \emph{not} meant to suggest that the algorithms and practical tweaks discussed above are always doomed. %, or that they comprise the single point of failure in \ac{GAN} training.
However, we do believe that they comprise an important cautionary tale to the effect that, in min-max problems,
\emph{convergence does not imply optimality} \textendash\ or even \emph{stationarity}.



\newpage  %% for ease of detecting page limits

==> relatedwork.tex <==
%----------------------------------------------------------------------
%%% RELATED
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


\para{Further related work} Our algorithmic framework applies to the majority of \emph{first-order} \cite{yadav2017stabilizing, GBVV+19, gidel2019negative, mokhtari2019unified, peng2020training} and \emph{scalable} second-order schemes\footnote{Second-order schemes involving Hessian-gradient multiplications can be scalable \cite{pearlmutter1994fast}, but inverting a Hessian is practically infeasible.} \cite{mescheder2017numerics, balduzzi2018mechanics}.
Nonetheless, we will omit algorithms with complicated feedback structures (such as best-response \cite{jin2019local, naveiro2019gradient}), or other tweaked min-max formulations such as mixed Nash \cite{hsieh2019finding, domingo2020mean} or Hidden Bilinear Games \cite{FVP19a}. We will also ignore finite games \cite{vNM44} since they bear relatively little consequences to our target applications in deep learning.

%When $\minvars, \maxvars$ are simplices and $\minmax$ is bilinear, \eqref{eq:minmax} reduces to the classical finite-strategy zero-sum games \cite{vNM44}. Since simplex constraints bear little consequences to our target applications in deep learning, we will omit this line of study.

Our analysis tools are deeply rooted in the theory of dynamical systems \cite{Ben99, BH96}, which have been exploited in the study of non-convex optimization \cite{lee2016gradient, panageas2017gradient}. However, to the best of our knowledge, with the sole exception of \cite{mazumdar2020gradient}, they have not been applied to generic non-convex non-concave \eqref{eq:minmax}. The focus of \cite{mazumdar2020gradient} is on convergence to critical points, which is less general than our framework, and the authors of \cite{mazumdar2020gradient} do not establish the connection to existing algorithms.

Upon the completion of this work, a very recent preprint \cite{letcher2020impossibility} studying non-convex non-concave games appeared on \texttt{arXiv}. The major distinction is that \cite{letcher2020impossibility} focuses on impossibility of \emph{desirable convergence} by providing counterexamples, whereas our theory proves \emph{undesirable convergence}, a strengthened negative result. Moreover, the framework of \cite{letcher2020impossibility} was only applied to gradient descent, whereas our template in \cref{sec:algorithms} subsumes many of the existing methods.

%there are major distinctions between \cite{letcher2020impossibility} and our work. First, \cite{letcher2020impossibility} disproves convergence to critical points while avoiding strict maxima by considering counterexamples, whereas we focus on the more general ICT sets. Second, the author only applied the results to gradient descent, whereas we incorporate many other existing methods; \cf \cref{sec:algorithms}. Finally, 
%proves that certain algorithms can exhibit non-convergent behavior by providing examples, while we 
%\section{Related work}

%\PM{This is a test citation of \citet{Ben99} and another for \citet{BH96}.
%This is some more related work, with a test citation of \citet{HS03}.}

%We focus on non-convex non-concave (i.e. non-monotone) games, thus omitting all literature that assume convexity/concavity. However, since bilinear games are used by many existing work to motivate new algorithms, we include them below.

%We ignore games with finite strategies such as in \cite{bailey2019fast,cheung2019vortices}. We also omit mixed NE algorithms such as \cite{domingo2020mean, hsieh2019finding, kamalaruban2020robust}.


%\para{Dynamical Systems in games:}
%argue that discrete and continuous systems have the same convergence behavior.


%bilinear 


%\para{Scalable Second-Order Algorithms:} Not involving inversion of Hessian or Jacobian
%%\cite{raghunathan2019game}: Gradient-based Nikaido-Isoda Function
%
%\cite{mescheder2017numerics}: consensus optimization
%
%\cite{balduzzi2018mechanics}: symplectic gradient adjustment
%%\para{Local Approaches}
%
%\cite{abernethy2019last}: Hamiltonian descent

%{\citet{wang2019solving}: Follow the Ridge}
%Based on the implicit function theorem (and therefore a \emph{local} argument), the authors propose a new algorithm called the Follow-the-Ridge (FR). The authors prove that, under certain conditions, all strictly stable fixed points of FR are local minimax and vice versa.
%
%This is a ``truly'' second-order algorithm in that it requires to invert the Hessian of the second player, and hence is not scalable.

%\PM{Very good, don't have to deal with it.}

%\begin{align*}
%x_{t+1} &= x_t - \eta_x \nabla_x \Phi(x_t, y_t), \\
%y_{t+1} &= y_t + \eta_y \nabla_y \Phi(x_t,y_t) + \eta_x \nabla^2_{yy} \Phi(x_t,y_t)^{-1}  \nabla^2_{yx} \Phi(x_t,y_t)\nabla_x \Phi(x_t, y_t)
%\end{align*}

%{\citet{raghunathan2019game}: Gradient-based Nikaido-Isoda Function}
%The paper proposes a local variant of the Nikaido-Isoda function called Gradient-based Nikaido-Isoda Function (GNI). The authors prove that gradient descent on GNI is locally stable on fixed points.

%Gradient descent on GNI is a second-order method. The authors propose a modified first-order algorithm that (under quite strong assumptions) retains the same convergence. 

%\subsubsection{\citet{mazumdar2019finding}: Local Symplectic Surgery}
%The authors take advantage of the two-player zero-sum structure and construct a two-time scale algorithm such that local Nash are the only attracting fix points and hence is locally stable.
%
%Note that this applies only to two-player zero-sum. In addition, this is a second-order method.
%
%\PM{Why the hell ``surgery''? Because they saw Hamilton and Perelman and thought it was sexy? Grrrr\dots}
%
%\YPH{How about we rename limit cycles to ``pseudo-periodic convergence with trivial fundamental group in the Poincar\'e sense''?}

%\subsubsection{\citet{liu2019towards}}
%The paper proves that, under the assumption that Minty Variational Inequality has a solution, a new adaptive version of OMD (called OAdagrad) attains faster rate than SOMD.
%
%\PM{This is from one of your favorite authors? Or one of Ahmet's? Or both?}
%\YPH{Ahmet's love of life.}


%\subsubsection{\citet{mazumdar2020gradient}} 
%The authors exploit the dynamical system viewpoint of learning in continuous games. In particular they invoke \citet{Ben99} to argue that discrete and continuous systems have the same convergence behavior.
%
%They focus on characterizing the relationship between locally asymptotically stable equilibria and local Nash equilibria.
%
%\PM{Ok, so we'll probably get those as reviewers. I saw this paper float around a couple of weeks ago but haven't read it yet \textendash\ will do\dots}
%\YPH{Don't waste your time on this paper... They said something like local NE is contains locally stable equilibria or whatever and that's it.}


%\subsubsection{\citet{nie2019towards}: Jacobian Regularization}
%The authors propose a method to regularize the Jacobian so that the training dynamics of GANs is locally more (numerically) stable.
%
%\PM{Ok.}


%\subsubsection{\citet{zhang2019policy}}
%The authors focus on zero-sum linear quadratic (LQ) games. They develop three projected ``nested-gradient'' methods that are guaranteed to converge to Nash equilibria of LQ games.
%
%\PM{Ooook?}

%\subsubsection{\citet{jin2019local}}
%This paper proposes a local optimality measure called ``local minimax'', and proves that all stable limit points of GDA are (under some conditions) local minimax.
%
%\PM{This is the paper we were talking about, right? I think we can safely ignore papers requiring access to an optimization oracle (even an approximate one).}
%
%\YPH{Yes. They have two results, one with max oracles and the other invoking \cite{daskalakis2018limit}. We can safely subsume this paper into the discussion of \cite{daskalakis2018limit}. }


%\subsubsection{\citet{daskalakis2018limit}}
%The authors show that (optimistic) GDA avoid unstable critical points for almost all initialization.
%
%\PM{Unstable in what sense? [I mean, relative to which dynamics/definition/notion?]}
%\YPH{Jacobians at the equilibria have spectral radius $\leq 1$. The (discrete) dynamics are GDA and optimistic GDA.}


%\subsubsection{\citet{berard2019closer}}
%The paper empirically shows that training of GANs exhibits significant rotations around local stable stationary points. {\color{red}(!!! Limit cycles ???)} In addition, the authors provide empirical evidence that GAN training converges to a stable stationary point which is a saddle point for the generator (not a minimum) while still achieving excellent performance.
%
%\PM{Ok, I'd need to understand this better (this is a dick thing to say but, in general, I'm a bit wary when it comes to statements from Gidel and company).}
%
%\YPH{I thought it's an agreement of us that the Simon factory manufactures things that are homotopic to shit. That being said, this paper is largely empirical and hence at least there's more credibility. }

%\subsubsection{\citet{mescheder2018training}}
%The paper investigates the local convergence behavior of various GANs and regularization.
%
%\PM{OK.}

%\subsubsection{\citet{liang2019interaction}}
%The paper analyzes the local convergence of bilinear games of various algorithms.
%
%\PM{Ok!}

%\subsubsection{\citet{nagarajan2017gradient}}
%The paper shows that, under certain assumptions, GDA for traditional GANs is locally asymptotically stable. Moreover, the authors show that this is not the case for WGANs.
%
%\PM{Hmmm\dots were you able to figure out the assumptions?}
%\YPH{The assumptions are on data distributions and less so on the loss function. We can safely ignore this.}


%The authors claim that WGANs can have \emph{limit cycles}. However, by inspecting their example, one finds that the authors prove that there exist ``periodic orbits'' (such as in bilinear games) under specific initialization. This is quite different from our example, where we construct global limit cycles that attract \emph{all} initialization.
%
%\PM{Ok \textendash\ would still need to understand this in detail though\dots}
%\PM{They really prove something in a real WGAN model?}
%
%\YPH{It is a toy WGAN with polynomial activation. See Appendix E in their arxiv version.}



%\subsubsection{\citet{heusel2017gans}}
%The paper focuses on local NE, and proposes a two-time scale discretization of the dynamical systems. 
%
%\YPH{It is perhaps worth noting that the paper invokes Borkar's theory \cite{borkar1997stochastic}. In addition, it contains a continuous-time dynamics for ADAM.}
%\PM{Yes, Borkar is the go-to ref for two-time-scale methods. However, isn't there another paper by Mazumdar in the list doing sth similar?}
%\YPH{Their algorithms seem different although both invoke Borkar's theory.}


%\subsubsection{\citet{schafer2019competitive, schafer2019implicit}: Competitive Gradient Descent}
%The authors propose a new algorithm, called the competitive gradient descent (CGD), that builds on a local bilinear approximation of the game. Hence, at best, CGD retains local properties of the game.
%
%This is a second-order method.
%
%\PM{Ok. \href{https://www.youtube.com/watch?v=bT90D0GKZRM}{Bye Felicia \smiley}}
%
%\YPH{Didn't know that you're a meme lord.}

%\subsubsection{\citet{mescheder2017numerics}: Consensus Optimization}
%The authors analyze the local convergence theory based on the eigenvalues of the Jacobian. The authors further propose a new optimization, called the ``consensus optimization'' which mixes GAD with Hamiltonian descent.
%
%\YPH{I think this is a perfect example to make our point: People naively believe that if GAD handles the potential part and Hamiltonian descent handles the solenoidal part, then mixing them handles both. Our theory says that this is far from the truth.}
%
%\PM{Very good!}

%\subsubsection{\citet{peng2020training}: Centripetal Acceleration}
%The authors propose a generalization of OMD, the centripetal acceleration, that converges for bilinear games.
%
%\PM{Isn't ``centripetal'' just another name for ``optimistic''?}
%
%\YPH{Yes... They consider $\alpha\nabla_t + \beta(\nabla_t - \nabla_{t-1})$ and call the second term centripetal acceleration (so $\alpha = \beta$ goes back to OMD). By the way \citet{mokhtari2019unified} also analyze such generalization. }

%\subsubsection{\citet{adolphs2019local}: Extreme Curvature Exploitation}
%The paper proposes a method, called the Extreme Curvature Exploitation, to escape undesired stable stationary points.
%
%This is a second-order algorithm.
%
%\PM{V. good, you know what I'm gonna say: \href{https://www.youtube.com/watch?v=bT90D0GKZRM}{Bye Felicia \smiley}}


%
%\subsubsection{\citet{azizian2019tight}}
%The paper provides a unified analysis for GD, OMD, EG, and CO on bilinear games.
%
%\PM{Interesting \textendash\ what do they show?}
%
%\YPH{They show that the author list is [Azizian-Mitliagkas-Lacoste-Julien-Gidel] and I stopped reading after that.}


%\subsubsection{\citet{mokhtari2019unified}}
%Based on the proximal point approach, the paper proposes an analysis framework for EG and OMD on bilinear games (and also strongly monotone games). 
%
%\PM{Ok.}

%\subsubsection{\citet{gidel2019negative}: Negative Momentum}
%The authors propose a new algorithm, motivated by the negative momentum, and prove that it converges for bilinear games.
%
%\PM{``Negative momentum'' meaning what exactly, did you figure this out?}
%
%\YPH{ $x_{t+1} =\textup{gradient step} + \beta (x_{t}  -x_{t-1} ) $, the second term is called ``negative momentum'' since it negates the momentum \`a la Polyak/Nesterov.}



%\subsection{Global Approaches}
%
%\subsubsection{\citet{balduzzi2018mechanics}}
%The paper classifies the games into potential and Hamiltonian games. The authors claim that Hamiltonian games are purely rotational, and they propose an algorithm, called the symplectic gradient adjustment, to combat the non-convergence of GDA.
%
%\PM{If ``symplectic gradient adjustment'' is what I think it is (descent of gradient norm squared), it performs \textbf{horribly} in our example. It converges to points that have nothing to do with equilibrium (just the gradients are small because they're near a periodic orbit).}
%
%\YPH{See below. I also forgot to add that symplectic gradient adjustment is a second-order method.}


%\subsubsection{\citet{abernethy2019last}: Gradient descent on Hamiltonian}
%The main result of the paper states that if a game is sufficiently bilinear and all critical points of the objective are global min-maxes, then Hamiltonian descent (HD) converges to optima . The authors also prove that mixing GDA with HD (known as ``consensus optimization'' \cite{mescheder2017numerics}) also converges with the same guarantee.

%This is a second-order method.
%
%\PM{``All critical points of the objective are global min-maxes''. Also, I smell a rat, let's discuss this in detail\dots}


%Let $\mathcal{H} \coloneqq \frac{1}{2} \|   \nabla \Phi \|^2$. Define the Hamiltonian descent dynamics by
%\begin{equation}
%\label{eq:hamiltonian_descent_dynamics}
%\dot{z} = -\nabla \mathcal{H}(z), \quad z = \begin{bmatrix}
%x \\
%y
%\end{bmatrix}.
%\end{equation}Hamiltonian descent is the Euler discretization of \eqref{eq:hamiltonian_descent_dynamics}. We can also define the ``consensus dynamics'' by
%\begin{equation}
%\label{eq:consensus_dynamics}
%\dot{z} = -   \begin{bmatrix}
%\nabla_x \Phi \\
%-\nabla_y \Phi
%\end{bmatrix} - \lambda\nabla \mathcal{H}(z)
% \end{equation}where $\lambda >0$ is a mixture parameter. Consensus optimization \cite{mescheder2017numerics} is the Euler discretization of \eqref{eq:consensus_dynamics}.



%Let $A$ be the asymmetric part of the game Hessian $\begin{bmatrix}
%\nabla^2_{xx} \Phi &\nabla^2_{xy}\Phi \\
%-\nabla^2_{yx} \Phi & -\nabla^2_{yy} \Phi
%\end{bmatrix}.$ Then symplectic gradient adjustment \cite{balduzzi2018mechanics} amounts to
%\begin{equation}
%\label{eq:symplectic_gradient_adjustment}
%\dot{z} = -   \begin{bmatrix}
%\nabla_x \Phi \\
%-\nabla_y \Phi
%\end{bmatrix} - \lambda A^\top \begin{bmatrix}
%\nabla_x \Phi \\
%-\nabla_y \Phi
%\end{bmatrix}.
% \end{equation}
%
%\YPH{I do think symplectic gradient adjustment makes more sense than Hamiltonian descent in the following sense. Notice that HD does not care about the sign of gradients, which means it is the same for $\min\max, \max\max, \max\min, \min\min$. This is of course very weird. At lest symplectic gradient adjustment somehow takes care of the sign. }



%\subsubsection{\citet{bailey2019finite}}
%The authors show that for a bilinear game, alternating GD results in cycles.
%
%\PM{Whoop-dee-whoop, stop the presses\dots}
%\YPH{No joke I got headache reading this paper.}

%\subsubsection{\citet{mertikopoulos2018optimistic}}
%The paper proposes a property called ``coherence'', and proves the convergence of MD and OMD under coherence.
%
%\PM{Whoop-dee-whoop, stop the presses\dots}
%
%\YPH{I know, I sent Trump the paper and told him that he needs to be coherent.}
%
%
%\subsubsection{\citet{naveiro2019gradient}}
%The authors propose to solve Stackelberg games by a double-loop algorithm that corresponds to approximate best-response dynamics. The convergence is proved based on an approximate monotone property (Condition 2 in \textbf{Proposition 1}).
%
%\PM{Ok, haven't seen this paper, would need to read/understand more about this.}
%\YPH{I say we can safely ignore this paper.}

